The Batik-plays-Mozart Corpus: Linking Performance to Score to Musicological Annotations

We present the Batik-plays-Mozart Corpus, a piano performance dataset combining professional Mozart piano sonata performances with expert-labelled scores at a note-precise level. The performances originate from a recording by Viennese pianist Roland Batik on a computer-monitored B\"osendorfer grand piano, and are available both as MIDI files and audio recordings. They have been precisely aligned, note by note, with a current standard edition of the corresponding scores (the New Mozart Edition) in such a way that they can further be connected to the musicological annotations (harmony, cadences, phrases) on these scores that were recently published by Hentschel et al. (2021). The result is a high-quality, high-precision corpus mapping scores and musical structure annotations to precise note-level professional performance information. As the first of its kind, it can serve as a valuable resource for studying various facets of expressive performance and their relationship with structural aspects. In the paper, we outline the curation process of the alignment and conduct two exploratory experiments to demonstrate its usefulness in analyzing expressive performance.

==> tables/cad_distr_table.tex <==
\small
% \begin{tabular}{|l|l|l|l|l|lllll}
% \cline{1-5}
% \multirow{2}{*}{tempo class} & \multirow{2}{*}{num pieces} & \multirow{2}{*}{num cadence labels} & authentic \% & \multirow{2}{*}{of which downbeat} &                   &  &  &  &  \\ \cline{4-4}
%                              &                             &                                     & half \%      &                                    &                   &  &  &  &  \\ \cline{1-5}
% \multirow{2}{*}{adagio}      & \multirow{2}{*}{4}          & \multirow{2}{*}{64}                 & 55.91        & 52.98                              & \multirow{2}{*}{} &  &  &  &  \\
%                              &                             &                                     & 44.09        & 29.17                              &                   &  &  &  &  \\ \cline{1-5}
% \multirow{2}{*}{andante}     & \multirow{2}{*}{8}          & \multirow{2}{*}{103}                & 78.71        & 86.31                              & \multirow{2}{*}{} &  &  &  &  \\
%                              &                             &                                     & 29.17        & 42.67                              &                   &  &  &  &  \\ \cline{1-5}
% \multirow{2}{*}{allegretto}  & \multirow{2}{*}{4}          & \multirow{2}{*}{123}                & 46.36        & 73.67                              & \multirow{2}{*}{} &  &  &  &  \\
%                              &                             &                                     & 53.64        & 50.61                              &                   &  &  &  &  \\ \cline{1-5}
% \multirow{2}{*}{allegro}     & \multirow{2}{*}{16}         & \multirow{2}{*}{352}                & 64.94        & 85.66                              & \multirow{2}{*}{} &  &  &  &  \\
%                              &                             &                                     & 35.06        & 61.06                              &                   &  &  &  &  \\ \cline{1-5}
% \multirow{2}{*}{menuetto}    & \multirow{2}{*}{2}          & \multirow{2}{*}{36}                 & 65.00        & 92.10                              & \multirow{2}{*}{} &  &  &  &  \\
%                              &                             &                                     & 35.00        & 100.00                             &                   &  &  &  &  \\ \cline{1-5}
% \multirow{2}{*}{presto}      & \multirow{2}{*}{2}          & \multirow{2}{*}{48}                 & 67.15        & 100.00                             & \multirow{2}{*}{} &  &  &  &  \\
%                              &                             &                                     & 32.86        & 100.00                             &                   &  &  &  &  \\ \cline{1-5}
% \multirow{2}{*}{total}       & \multirow{2}{*}{36}         & \multirow{2}{*}{708}                & 60.88        & 78.89                              &                   &  &  &  &  \\
%                              &                             &                                     & 39.12        & 61.37                              &                   &  &  &  &  \\ \cline{1-5}
% \end{tabular}


\small
\begin{tabular}{|l|l|l|l|lllll}
\cline{1-4}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}tempo \\ class\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}cadence \\ labels\end{tabular}} & authentic \% & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}of which \\ downbeat\end{tabular}} &  &  &  &  &  \\ \cline{3-3} &     & half \% & &  &  &  &  &  \\ 
\cline{1-4} \multirow{2}{*}{adagio} & \multirow{2}{*}{64} & 55.91      & 52.98 & \multirow{2}{*}{} &  &  &  &  \\ & & 44.09 & 29.17 & &  &  &  &  \\ 
\cline{1-4} \multirow{2}{*}{andante}  & \multirow{2}{*}{103} & 78.71 & 86.31 & \multirow{2}{*}{} &  &  &  &  \\ & & 29.17 & 42.67 & &  &  &  &  \\ 
\cline{1-4} \multirow{2}{*}{allegretto} & \multirow{2}{*}{123} & 46.36 & 73.67 & \multirow{2}{*}{} &  &  &  &  \\ & & 53.64 & 50.61 & &  &  &  &  \\ 
\cline{1-4} \multirow{2}{*}{allegro} & \multirow{2}{*}{352} & 64.94 & 85.66 & \multirow{2}{*}{} &  &  &  &  \\ & & 35.06 & 61.06 & &  &  &  &  \\ 
\cline{1-4} \multirow{2}{*}{menuetto} & \multirow{2}{*}{36} & 65.00 & 92.10 & \multirow{2}{*}{} &  &  &  &  \\ & & 35.00 & 100.00 & &  &  &  &  \\ 
\cline{1-4} \multirow{2}{*}{presto} & \multirow{2}{*}{48} & 67.15 & 100.00 & \multirow{2}{*}{} &  &  &  &  \\ & & 100.00 & 100.00 &  &  &  &  \\

\cline{1-4} \multirow{2}{*}{total} & \multirow{2}{*}{708} & 60.88 & 78.89 & &  &  &  &  \\ &        & 39.12 & 61.37 & &  &  &  &  \\ \cline{1-4}
\end{tabular}
